Application of accelerated fixed-point algorithms to hydrodynamic well-fracture coupling

The coupled simulations of dynamic interactions between the well, hydraulic fractures and reservoir have significant importance in some areas of petroleum reservoir engineering. Several approaches to the problem of coupling between the numerical models of these parts of the full system have been developed in the industry in past years. One of the possible approaches allowing formulation of the problem as a fixed-point problem is studied in the present work. Accelerated Anderson's and Aitken's fixed-point algorithms are applied to the coupling problem. Accelerated algorithms are compared with traditional Picard iterations on the representative set of test cases including ones remarkably problematic for coupling. Relative performance is measured, and the robustness of the algorithms is tested. Accelerated algorithms enable a significant (up to two orders of magnitude) performance boost in some cases and convergent solutions in the cases where simple Picard iterations fail. Based on the analysis, we provide recommendations for the choice of the particular algorithm and tunable relaxation parameter depending on anticipated complexity of the problem.

==> tab/slugging_dt150.tex <==
%\begin{tabular}{|l|l|rrr|rrr|rrr|}
\begin{tabular}{|l|l|n{5}{1}n{5}{1}n{5}{1}|n{5}{1}n{5}{1}n{5}{1}|n{5}{1}n{5}{1}n{5}{1}|}
\bottomrule
     & Alg. & \multicolumn{3}{|l|}{ATK} & \multicolumn{3}{l}{FPI} & \multicolumn{3}{|l|}{TPA} \\
     & $\beta$ &   0.1 &   0.5 &   1.0 &    0.1 &    0.5 &    1.0 &    0.1 &   0.5 &   1.0 \\
\cline{2-11}
$c,\ 1/64''$ & $\theta,\ ^\circ$ &       &       &       &        &        &        &        &       &       \\
\cline{1-11}
\multirow{3}{*}{15.0} & -5.0 &  4465 &  4210 &  4793 &  60123 &  10680 &  10353 &  31373 &  5998 &  4924 \\
     &  0.0 &  3700 &  4707 &  4246 &  60395 &   9685 &   9393 &  19763 &  4737 &  3741 \\
     &  5.0 &  3545 &  4496 &  4003 &  60739 &   9990 &   8918 &  29777 &  6075 &  4436 \\
\cline{1-11}
\multirow{3}{*}{40.0} & -5.0 &  3627 &  3680 &  3624 &  62742 &   9746 &   3550 &  30075 &  5979 &  3682 \\
     &  0.0 &  3584 &  3608 &  3601 &  62591 &   9727 &   3453 &  29749 &  5988 &  3628 \\
     &  5.0 &  3507 &  3527 &  3531 &  62697 &   9760 &   3455 &  29040 &  5738 &  3611 \\
\cline{1-11}
\multirow{3}{*}{60.0} & -5.0 &  4749 &  4430 &  4668 &  65458 &  10614 &   4352 &  28009 &  6576 &  4392 \\
     &  0.0 &  3670 &  3722 &  3679 &  63312 &   9815 &   3608 &  27389 &  6002 &  3704 \\
     &  5.0 &  3620 &  3587 &  3612 &  62300 &   9680 &   3514 &  27494 &  5819 &  3630 \\
\cline{1-11}
{\bf Avg.} &     &  3829 &  3996 &  3973 &  62261 &   9966 &   5621 &  28074 &  5879 &  3972 \\
\toprule
\end{tabular}


==> tab/slugging_dt20.tex <==
%\begin{tabular}{|l|l|rrr|rrr|rrr|}
\begin{tabular}{|l|l|n{5}{1}n{5}{1}n{5}{1}|n{6}{1}n{5}{1}n{5}{1}|n{6}{1}n{5}{1}n{5}{1}|}
\cline{1-11}
     & Alg. & \multicolumn{3}{l|}{ATK} & \multicolumn{3}{l|}{FPI} & \multicolumn{3}{l|}{TPA} \\
     & $\beta$ &    0.1 &    0.5 &    1.0 &     0.1 &    0.5 &    1.0 &     0.1 &    0.5 &    1.0 \\
\cline{2-11}
$c, 1/64''$ & $\theta,\ ^\circ$ &        &        &        &         &        &        &         &        &        \\
\cline{1-11}
\multirow{3}{*}{15.0} & -5.0 &  12872 &  12950 &  12858 &  405675 &  62659 &  14179 &  129817 &  26687 &  13208 \\
     &  0.0 &  13173 &  13243 &  13284 &  410835 &  63855 &  14188 &  169768 &  25840 &  13164 \\
     &  5.0 &  13217 &  13210 &  13226 &  410930 &  63750 &  14398 &  125375 &  27234 &  13199 \\
\cline{1-11}
\multirow{3}{*}{40.0} & -5.0 &  15830 &  15791 &  15820 &  431409 &  66709 &  15692 &  146306 &  30667 &  16132 \\
     &  0.0 &  15501 &  15539 &  15535 &  429591 &  66685 &  15648 &  155729 &  30924 &  16137 \\
     &  5.0 &  15568 &  15637 &  15576 &  429429 &  66969 &  15739 &  151272 &  33076 &  16123 \\
\cline{1-11}
\multirow{3}{*}{60.0} & -5.0 &  16787 &  16730 &  16734 &  462578 &  71354 &  16489 &  136651 &  31470 &  16421 \\
     &  0.0 &  16488 &  16492 &  16471 &  455892 &  70083 &  16199 &  152419 &  31293 &  16420 \\
     &  5.0 &  16481 &  16438 &  16421 &  456655 &  70201 &  16180 &  155762 &  32589 &  16270 \\
\cline{1-11}
{\bf Avg.} &     &  15101 &  15114 &  15102 &  432554 &  66918 &  15412 &  147011 &  29975 &  15230 \\
\cline{1-11}

\end{tabular}


==> tab/tpa20.tex <==
\begin{tabular}{llrrrrrrrrr}
\toprule
    & Choke, 1/64'' & \multicolumn{3}{l}{15.0} & \multicolumn{3}{l}{40.0} & \multicolumn{3}{l}{60.0} \\
    & Inclination, $^\circ$ &    -5.0 &     0.0 &     5.0 &    -5.0 &     0.0 &     5.0 &    -5.0 &     0.0 &     5.0 \\
Algorithm & Relaxation factor &         &         &         &         &         &         &         &         &         \\
\midrule
\multirow{6}{*}{TPA} & 0.10 &  129817 &  169768 &  125375 &  146306 &  155729 &  151272 &  136651 &  152419 &  155762 \\
    & 0.25 &   45307 &   54477 &   48064 &   59681 &   64448 &   64967 &   58403 &   60643 &   62523 \\
    & 0.50 &   26687 &   25840 &   27234 &   30667 &   30924 &   33076 &   31470 &   31293 &   32589 \\
    & 0.75 &   18901 &   16813 &   19005 &   20311 &   19931 &   21324 &   21658 &   21362 &   21481 \\
    & 0.95 &   13347 &   13561 &   13246 &   16460 &   16695 &   16832 &   17257 &   16970 &   16925 \\
    & 1.00 &   13208 &   13164 &   13199 &   16132 &   16137 &   16123 &   16421 &   16420 &   16270 \\
\bottomrule
\end{tabular}

